Physics at the CLIC Multi-TeV Linear Collider

This report summarizes a study of the physics potential of the CLIC e+e- linear collider operating at centre-of-mass energies from 1 TeV to 5 TeV with luminosity of the order of 10^35 cm^-2 s^-1. First, the CLIC collider complex is surveyed, with emphasis on aspects related to its physics capabilities, particularly the luminosity and energy, and also possible polarization, \gamma\gamma and e-e- collisions. The next CLIC Test facility, CTF3, and its R&D programme are also reviewed. We then discuss aspects of experimentation at CLIC, including backgrounds and experimental conditions, and present a conceptual detector design used in the physics analyses, most of which use the nominal CLIC centre-of-mass energy of 3 TeV. CLIC contributions to Higgs physics could include completing the profile of a light Higgs boson by measuring rare decays and reconstructing the Higgs potential, or discovering one or more heavy Higgs bosons, or probing CP violation in the Higgs sector. Turning to physics beyond the Standard Model, CLIC might be able to complete the supersymmetric spectrum and make more precise measurements of sparticles detected previously at the LHC or a lower-energy linear e+e- collider: \gamma\gamma collisions and polarization would be particularly useful for these tasks. CLIC would also have unique capabilities for probing other possible extensions of the Standard Model, such as theories with extra dimensions or new vector resonances, new contact interactions and models with strong WW scattering at high energies. In all the scenarios we have studied, CLIC would provide significant fundamental physics information beyond that available from the LHC and a lower-energy linear e+e- collider, as a result of its unique combination of high energy and experimental precision.

==> Chap6/check.tex <==
In Fig.~\ref{lh5}, we show the total cross-Section versus $M_{W_H}$ 
at the CLIC energies, 3 and 5~TeV, for $\cot\theta~=~1$.  
The cross section grows when the mass increases because of the less
and less severe propagator suppression $1/(s-M_{Z_H})^2$, until
it is cut off by the threshold kinematics.
%fig30
\begin{figure}[tb]%[htbp] %[tb]
\centerline{\includegraphics[scale=0.71]{Chap6/lh5.ps}}
\caption{Total cross section for $\ee\to WW_H$ production versus its
mass $M_{W_H}$ at the CLIC energies $E_{c.m.}$~=~3 and 5~TeV.
Both charge states $W^\pm~W_H^\mp$ have been included.}
    \label{lh5}
\end{figure}

Generically, the mass and coupling of $W_H$ depend on $\cot\theta$,
the mixing parameter between the SM and new gauge groups 
$SU_L(2)$ and   $SU_H(2).$
Keeping the mass fixed at 1~TeV, we can explore the total cross section 
with respect to $\cot\theta$, as shown in~Fig.~\ref{cot}.  
%fig31
\begin{figure}[!hb]
\centerline{\includegraphics[scale=0.71]{Chap6/cot-clic.ps}}
\caption{Total cross section for $\ee\to WW_H$ production as a
function of gauge coupling mixing parameter $\cot\theta$ for
$M_{W_H}$~=~1~TeV} 
\label{cot}
\end{figure}

Once $W_H$ is produced, it can decay to SM particles, either 
fermion pairs or $WZ,\ WH$.  The branching fractions are given with
respect to the mixing parameter $\cot\theta$, as in~Fig.~\ref{brwh}.  
The decay channels  to fermions are dominant, asymptotically 1/4 for
the three generations of leptons or one generation of quarks,  
for most of the paramter space.
For a value of $\cot\theta<$~0.4, $W_H\to WH, WZ$ decay modes become more 
important, comparable to fermionic channels, as shown in~Fig.~\ref{brwh}.  
The production rate for the signal is still quite sizeable once above
the kinematical threshold, and likely above the SM backgrounds.
%fig32
\begin{figure}[tb]
%\centerline{\includegraphics[scale=1]{Chap6/brWH.ps}}
\centerline{\includegraphics[scale=0.9]{Chap6/brWH.ps}}
    \caption{Branching fractions for $W_H$ decay to SM particles}
    \label{brwh}
\end{figure}

In summary, once above the kinematical threshold, the heavy
gauge boson production at the CLIC energies can be substantial.
The threshold behaviour can determine its mass accurately, and the 
cross section rate will measure the coupling strength $\cot\theta$.



\subsection{Fourth Family}

The mass and mixing patterns of the fundamental fermions are among the
most mysterious aspects of particle physics today. The number of fermion
generations is not fixed by the SM. It is intriguing that
flavour democracy may hint at the existence of a fourth SM family (see
\cite{Sultansoy,Arik} and references therein), and its possible existence
is a fundamental question on which CLIC can cast new light. In order to
avoid violation of partial-wave unitarity, the masses of new quarks and
leptons should be smaller than about 1~TeV~\cite{Chanowitz}. Therefore,
CLIC with 1--3~TeV centre-of-mass energy will give the opportunity to
measure the fourth-SM-family fermions and quarkonia in detail.

Fourth-family quarks, if they exist, will be copiously produced at the
LHC~\cite{Arik2,ATLAS} if their masses are less than $1$~TeV.  Therefore,
any fourth-family quarks might be discovered at the LHC well before CLIC goes
into operation. The same is true for pseudoscalar quarkonia ($\eta_{4}$)
formed by the fourth-family quarks~\cite{Arik3}.  However, the observation of
the fourth-family leptons at the LHC is problematic because of the large
backgrounds from real $W$ and $Z$ boson production, both singly and in
pairs, that hide these heavy lepton signals~\cite{Barger}. Lepton
colliders will therefore be advantageous for the investigation of the
fourth-SM-family leptons and vector ($\psi_{4}$) quarkonia. The potential
of muon colliders was analysed in~Ref.~\cite{Ciftci}. In this section we
consider the production of the fourth-family fermions and quarkonia at CLIC,
starting with pair~production.

First we consider the $e^+e^-$ option of CLIC. The annihilation of
$e^{+}e^{-}$ is a classic channel to produce and study new heavy fermions,
because the cross sections are relatively large with respect to the
backgrounds~\cite{Barger}. The obtained cross section values for pair
production of the fourth-SM-family fermions with $m_{4}$~=~320~(640)~GeV
and the corresponding numbers of events per working year (10$^{7}$~s) are
given in Table~\ref{4_one} (Table~\ref{4_two}). %table
Event signatures are
defined by the mass pattern of the fourth family and the 4~$\times$~4
Cabibbo--Kobayashi--Maskawa (CKM) matrix. According to the scenario given
in~Ref.~\cite{Atag}, the dominant decay modes are $u_{4}\to b$ $W^{-}$,
$d_{4}\to t$ $W^{+}$, $l_{4}\to\nu_{\tau}W^{-}$ and
$\nu_{4}\to\tau^{-}W^{+}$. The charged $l_{4}$ lepton will have a
clear signature at CLIC. For example, if the produced $W^{\pm}$ bosons
decay leptonically, one has two acoplanar opposite-charge leptons and
large missing energy. Pair production of the neutral $\nu_{4}$ leptons
will lead to a more complicated event topology. In this case, $\tau$
tagging will be helpful for the identification of the events. Indeed, the
produced $\tau$ leptons will decay at a distance of 1--2~cm from the
interaction point, which can easily be measured by a vertex detector. In
addition, the polarization of electron and positron beams should help to
experimentally determine the axial and vector neutral-current coupling
constants of the fourth-family fermions.
%
\input{Chap6/table11.tex}
\input{Chap6/table12.tex}

Next we consider the $\gamma\gamma$ option~\cite{Ginzburg1,Ginzburg2,Telnov}
of CLIC. The fourth-SM-family quarks and charged
leptons will also be copiously produced at $\gamma\gamma$ machines. For
$\sqrt{s_{ee}}$~=~1~TeV (3~TeV), which corresponds to 
$\sqrt{s_{\gamma\gamma}}^{\max}$~=~0.83$\sqrt{s_{ee}}$~=~0.83~TeV
(2.5~TeV), the obtained cross section values 
and  number of events per year are presented in Table~\ref{4_one}
(Table~\ref{4_two}). 

Next we discuss quarkonium production. The condition to form 
$(Q\overline{Q})$ quarkonia states with new
heavy quarks is $m_{Q}\leq$~(125~GeV)~$|V_{Qq}|^{-2/3}$,
where $q=d,s,b$ for $Q=u_{4}$ and $q=u,c,t$ for $Q=d_{4}$~\cite{Bigi}.
Unlike the $t$ quark, the fourth-family quarks will form quarkonia 
because $u_{4}$ and $d_{4}$ are almost degenerate and their decays are
suppressed by small CKM mixings~\cite{Celikel,Atag,Sultansoy}. Below,
we consider the resonance
production of $\psi_{4}$ quarkonia at $e^{+}e^{-}$ and $\eta_{4}$ quarkonia
at $\gamma\gamma$ options of CLIC.

Again we first consider the $e^{+}e^{-}$ option for CLIC.
The cross section for the formation of the fourth-family quarkonium is 
given
by the well-known relativistic Breit--Wigner equation
\begin{equation}
\sigma\left(  e^{+}e^{-}\to\left(  Q\overline{Q}\right)  \right)
=\frac{12\pi\left(  s/M^{2}\right)  \Gamma_{ee}\Gamma}{\left(  s-M^{2}\right)
^{2}+M^{2}\Gamma^{2}}\,,
\label{4_bir}
\end{equation}
where $M$ is the mass, $\Gamma_{ee}$ is the partial decay width to $e^{+}%
e^{-}$ and $\Gamma$ is the total decay width of the fourth-family 
quarkonium.
Using corresponding formulae from~\cite{Barger87} in the framework of 
the Coulomb
potential model, we obtain decay widths for the main decay modes of $\psi
_{4}(u_{4}\overline{u_{4}})$ and $\psi_{4}(d_{4}\overline{d_{4}})$, which are
given in Table~\ref{4_three}. One can see that the dominant decay mode for 
both $\psi_{4}(u_{4}\overline{u_{4}})$ and $\psi_{4}(d_{4}\overline{d_{4}})$
quarkonia is $\psi_{4}\to W^{+}W^{-}$. Other important decay modes 
are $\psi_{4}\to\gamma Z$ and $\psi_{4}\to\gamma H$.
%
\input{Chap6/table13.tex}

In order to estimate the number of produced quarkonium states, one should
take into account the luminosity distribution at CLIC, which is influenced
by the energy spread of electron and positron beams and beamstrahlung. In
our calculations we use the GUINEA-PIG simulation code~\cite{Schulte}. For
illustration, we assume that $m_{\psi_{4}}\simeq$~1~TeV. The estimated
event numbers per year for $\psi_{4}$ production, as well as 
$\psi_{4}\to\gamma H$ and $\psi_{4}\to ZH$ decay channels are
presented in Table~\ref{4_four}. In numerical calculations we use 
$\Delta E/E$~=~10$^{-2}$ for the beam energy spread. 
If $\Delta E/E$~=~10$^{-3}$ can be achieved, the corresponding numbers
will be enlarged by a factor of about 8. 
The $\gamma H$ decay mode of the $\psi_{4}(u_{4}\overline{u_{4}})$
quarkonium is promising for the study of Higgs boson properties,
especially if the energy spread of electron and positron beams of
about 10$^{-2}$ \ could be controlled to about 10$^{-3}$.
%
\input{Chap6/table14.tex}

Finally, we discuss again the $\gamma\gamma$ collider.
The pseudoscalar $\eta_{4}$ quarkonia formed by the fourth-SM-family 
quarks will be copiously produced at the LHC~\cite{ATLAS,Arik3}. Decay
widths for the main decay modes of 
$\eta_{4}(u_{4}\overline{u_{4}})$ and 
$\eta_{4}(d_{4}\overline{d_{4}})$ are given in Table~\ref{4_five}. 
From there, it is clear that the dominant decay
mode is $\eta_{4}\to ZH$. One can estimate the $\gamma\gamma
\to\eta_{4}$ production cross section by using 
the following relation~\cite{Gorbunov}:
\begin{equation}
\sigma\approx 50\,{\rm fb}(1+\lambda_{1}\lambda_{2})
\left( \frac{BR_{\gamma\gamma}}{4\times10^{-3}}\right)  
\left( \frac{\Gamma_{\rm tot}}{1\,{\rm MeV}}\right)  
\left( \frac{200\,{\rm GeV}}{M_{\eta}}\right)^{3}\,,
\end{equation}
where $BR_{\gamma\gamma}$ is the branching ratio of 
the $\eta_{4}\to\gamma\gamma$ decay mode, 
$\Gamma_{\rm tot}$ is the\ quarkonium total decay width
and $\lambda_{1,2}$ are helicities of the initial photons. 
Assuming $\lambda_{1}\lambda_{2}$~=~1, we obtain total event numbers
of $\eta_{4}$ produced per year as follows: 
900~$\eta_{4}(u_{4}\overline{u_{4}})$ and 
56~$\eta_{4}(d_{4}\overline{d_{4}})$. 
The corresponding numbers for $\eta_{4}\to ZH$ events are 610 and 38
events, respectively. The advantage of 
$\eta_{4}(u_{4} \overline{u_{4}})$ with respect to
$\eta_{4}(d_{4}\overline{d_{4}})$ is obvious.
%
\input{Chap6/table15.tex}

\subsection{Leptoquarks}

In the SM of electroweak and colour (QCD)
interactions, quarks and leptons appear as formally independent
components. However, the observed symmetry between the lepton and
quark sectors in the SM could be interpreted as a hint for common
underlying structures. If quarks and leptons are made of
constituents there should appear, at the scale of constituent binding
energies, new interactions among leptons and quarks.
Leptoquarks (LQs) are exotic particles carrying both lepton number
(L) and baryon number (B), which are colour (anti-)triplet, scalar or 
vector
particles that appear naturally in various unifying theories
beyond the SM. The interactions of LQs with the known particles
are usually described by an effective Lagrangian that satisfies
the requirement of baryon- and lepton-number conservation and
respects the $SU(3)_{C}~\times~SU(2)_{W}~\times~U(1)_{Y}$ symmetry
of the SM. There are nine scalar and nine vector leptoquark types
in the Buchm\"uller--R\"uckl--Wyler (BRW) classification~\cite{1}. The
scalar leptoquarks $(S,R)$ can be grouped into singlets
$(S_{0},\widetilde{S}_{0}),$ doublets
$(R_{1/2},\widetilde{R}_{1/2})$ and triplet $(S_{1}).$ Here, we
assume only the mass, and the couplings to right-handed and/or
left-handed leptons, denoted by $g_{\rm R}$ and $g_{\rm L}$, remain as
free parameters~\cite{2}. From the BRW effective interaction
Lagrangian~\cite{1} one can deduce the quantum numbers of scalar
leptoquarks given in Table~\ref{table1}.
%table16

The leptoquarks are constrained by different experiments. Direct limits on
leptoquark states are obtained from their production cross sections at
different colliders, while indirect limits are calculated from the bounds
on the leptoquark-induced four-fermion interactions in low-energy
experiments. The mass limits for scalar leptoquarks from single and pair
production, assuming electromagnetic coupling, are
$M_{LQ}>$~200~GeV~\cite{3} and $M_{LQ}>$~225~GeV~\cite{4}, respectively.

We have studied the potential of a CLIC-based $e\gamma$ collider to search
for scalar leptoquarks, taking into account both direct and resolved
photon processes. Scalar leptoquarks can be produced singly in $e\gamma$
collisions, via the process $e\gamma\to Sq$, where $S$ is any type
of scalar leptoquark ($S$ or $R$). At $e\gamma$ colliders, with a photon
beam produced by Compton backscattering~\cite{5}, the maximum $e\gamma$
centre-of-mass energy is about 91\% of the available energy. The projects
of CLIC~\cite{6} colliders will be working at $\sqrt{s_{e^{+}e^{-}}}$~=~1
TeV to $\sqrt{s_{e^{+}e^{-}}}$~=~3~TeV. Corresponding high-energy photon
beams can be obtained from the linacs with energies $\simeq$~415~GeV and
$\simeq$~1245~GeV for CLIC at these energies.

We have implemented the interactions between scalar leptoquarks, leptons
and quarks into the CompHEP program~\cite{comphep} with an internal photon
spectrum. The main contribution to the total cross section comes from the
$u$-channel quark-exchange diagram. For this reason, the total cross
Sections for the production of scalar leptoquarks $R_{1/2}$(--~5/3),
$S_{0}$(--~1/3) and $S_{1}$(--~1/3) practically coincide. This is also true
for $R_{1/2}$(--~2/3), $\widetilde {R}_{1/2}$(--~2/3), 
$\widetilde{S}_{0}$(--~4/3)
and $S_{1}$(--~4/3) type scalar leptoquarks.

The scalar leptoquarks can also be produced in $e\gamma$
collisions by resolved photon processes. In order to produce
leptoquarks in the resonant channel through the quark component of
the photon, we study the following signal for the scalar
leptoquark $S$ (or $R$), $e+q_{\gamma}\to S\to e+q$. 
For CLIC-based $e\gamma$ colliders, the total cross section
for resolved photon contribution is obtained by convoluting with
the back-scattered laser photon distribution and photon structure
function. The photon structure function consists of perturbative
point-like parts and hadron-like parts
$f_{q/\gamma}=f_{q/\gamma}^{\rm PL}+f_{q/\gamma}^{\rm HL}$~\cite{8}.
Since the contribution from the point-like part of the photon
structure function was already taken into account in the
calculation of the direct part, it was subtracted from
$f_{q/\gamma}$ to avoid double 
counting at the leading-logarithmic~level.

Both schemes can give comparable results for the production cross
Section. Therefore, we add their contribution to form the signal.
In this case, the total cross section for the production of scalar
LQs is $\sigma=\sigma_{\rm D}+\sigma_{\rm R}$, where $\sigma_{\rm D}$ and
$\sigma_{\rm R}$ denote the direct and resolved contributions to the
total cross section, respectively. The total cross sections
including both direct and resolved contributions are plotted in
Fig.~\ref{fig1} for CLIC-based $e\gamma$ colliders with
$\sqrt{s_{e^+e^-}}$~=~1~TeV. As can be seen from this figure, the
contribution from the resolved process is dominant for small
leptoquark masses and the direct contribution is effective for larger
masses up to the kinematical limit. Depending on the centre-of-mass 
energy, the resolved contribution decreases sharply beyond a
leptoquark mass value of about 70\% of the collider energy.
%
The direct contribution for a scalar leptoquark with $|Q|$~=~5/3 is
larger than the scalar leptoquark with $|Q$|~=~4/3. This can be
explained by the quark-charge dependence of the cross sections
for direct contributions. The coupling for the lepton--quark--leptoquark
vertex can be parametrized as $g_{LQ}=\sqrt{4\pi\alpha\kappa}$,
where $\kappa$ is a parameter.

\newpage
\input{Chap6/table16.tex}
\newpage
\input{Chap6/table17.tex}
\newpage

%fig33
\begin{figure}[t]
\includegraphics[
height=7cm, width=8cm ] {Chap6/lepto_fig1.eps}
\includegraphics[
height=7cm, width=8cm ] {Chap6/lepto_fig2.eps}\\
\centerline{(a)
$\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad$ (b)}
\caption{The direct (D) and resolved (R) contributions to the
cross section depending on scalar leptoquark mass $M_{LQ}$ at
$\sqrt{s_{e^+e^-}}$~=~1~TeV with LQs
charges a) $|Q|$~=~5/3~(1/3) and b) $|Q|$~=~4/3~(2/3).} 
\label{fig1}
\end{figure}

When a scalar leptoquark is singly produced at an $e\gamma$ collider, the
signal will be two jets and a charged lepton $2j+l$ ($S$ and $R$
leptoquarks), or two jets plus a neutrino $2j+\not\!p_{T}$ ($S$
leptoquarks). Since leptoquarks generate a peak in the invariant ($lj$)
mass distribution, singly-produced leptoquarks are easy to detect up to
mass values close to the kinematical limit. In the case of equal couplings
$g_{\rm L}=g_{\rm R}$, the branching ratios for $S_0$ can be obtained
as 2/3 for $LQ\to lq$ and 1/3 for $LQ\to \nu q$ channels.

In order to calculate the statistical significance $S/\sqrt{B}$ at each
mass value of a scalar leptoquark and for each decay channel, we need to
calculate also the relevant background cross sections. For the background
processes $e\gamma\to W^{-}\nu$ and $e\gamma\to Ze$, we
find the total cross sections 41.20~(49.48)~pb and 2.36~(0.49)~pb
at $\sqrt{s_{e^{+}e^{-}}}$~=~1~(3)~TeV, respectively. We multiply these
cross sections with the branching ratios for the corresponding channels.

For a $e\gamma$ collider with centre-of-mass energy
$\sqrt{s_{e^+e^-}}$~=~1~TeV and total luminosity 
$L$~=~10$^{5}$~pb$^{-1}$, the scalar leptoquarks of types
$S_{0},S_{1}^{0}$ and $R_{1/2}^{-1/2}$ can be
produced up to mass $M_{LQ}\approx$~900~GeV, and 
$R_{1/2}^{1/2},\widetilde{S}_{0},S_{1}^{-1},\widetilde{R}_{1/2}^{-1/2}$ 
up to $M_{LQ}\approx$~850~GeV in
the $2j+e$ channel. However, leptoquarks of types $S_{0},S_{1}^{0}$ can be
produced up to $M_{LQ}\approx$~850~GeV and $R_{1/2}^{1/2}$ up to 
$M_{LQ}\approx$~650~GeV in the $2j+\not \! p_{T}$ channel. For an $e\gamma$
collider with $\sqrt{s_{e^+e^-}}$~=~3~TeV and total
luminosity $L$~=~10$^{5}$~pb$^{-1}$, the scalar leptoquarks of type 
$S_{0},S_{1}^{0},R_{1/2}^{-1/2}$ could be produced up to mass 
$M_{LQ}\approx$~2600~GeV, types 
$\widetilde{R}_{1/2}^{-1/2},\widetilde{S}_{0},S_{1}^{-1}$ up to mass
$M_{LQ}\approx$~2500~GeV, type $R_{1/2}^{1/2}$ up to 
$M_{LQ}\approx$~2100~GeV in
the $2j+e$ channel; and scalar leptoquarks of type $R_{1/2}^{1/2}$ up to 700
GeV, $S_{0}$ up to 900~GeV and $S_{1}^{0}$ up to 1300~GeV in the
$2j+\not \! p_{T}$ channel. The total number of signal events and
statistical significance for these channels
are given in Tables~\ref{table2} and \ref{table3}.
%

To conclude: scalar leptoquarks can be produced in large numbers at
CLIC-based $e\gamma$ colliders. We have analysed the contributions from
direct and resolved photon processes to the total cross section. We
find that 
the latter contribution is important and cannot be ignored, especially for
small leptoquark masses. Looking at the final-state particles and their
signature in detectors, scalar leptoquarks of various types can be
identified easily.

\newpage
\input{Chap6/table18.tex}
\newpage

\subsection{Lepton-Size Measurements}

High-energy $e^+e^-$ scattering can also be used to study whether the
leptons have a finite size. Similar studies have been made in the past,
for example at LEP~\cite{Bourilkov:2000ap}. A model inspired by string
theory, which can lead to elastic ministrings, with finite size (dubbed
Nylons), has been proposed in~Ref.~\cite{lykken}.

In the presence of structure, annihilations to fermions $f$ will be
modified to become 
$\frac{d\sigma}{dQ^2}=(\frac{d\sigma}{dQ^2})_{\rm SM}F_e^2(Q^2)
F_f^2(Q^2)$, 
with $ F(Q^2)=1+\frac{1}{6}Q^2R^2$, where $R$
is an effective fermion radius. The current best limit on the radius $R_e$
of the electron comes from LEP, and is 
$R_e<$~2.8~$\times$~10$^{-17}$~cm (95~C.L.). For CLIC, the results for
$ee\to ee$, under the assumption 
that the $t$ channel dominates, for an angular cut on the scattered
electrons of $|\cos\theta|<$~0.9, and for a luminosity of 500~fb$^{-1}$,
are given in Table~\ref{sec6:nylons}. We see that a 5-TeV machine will
probe structures of dimensions a factor of 10 smaller than in the
present results from LEP~\cite{Bourilkov:2000ap}.
%
\input{Chap6/table19.tex}

\subsection{Excited Electrons}

The replication of three fermionic generations of known quarks and leptons
suggest, the possibility that they are composite structures made up of more
fundamental constituents. The existence of such quark and lepton
substructure leads one to expect a rich spectrum of new particles with
unusual quantum numbers. A possible signal of excited states of quarks and
leptons~\cite{9} as predicted by composite models~\cite{10} would supply
convincing evidence for a new substructure of matter. All composite models
of fermions have an underlying substructure that may be characterized by
a scale $\Lambda$. The absence of electron and muon electric dipole
moments implies that the excited leptons must have specific chiral
properties. A right-handed excited lepton should couple only to the
left-handed component of the corresponding lepton. Excited leptons may be
classified by $SU(2)~\times~U(1)$ quantum numbers, and they are assumed to
be both left- and right-handed weak isodoublets. In the effective
Lagrangian of~\cite{9}, the parameters $f$ and $f^{\prime }$ associated
with the gauge groups SU(2) and U(1) depend on compositeness dynamics and
describe the effective changes from the SM coupling constants $g$ and
$g^{\prime }$.

Experimental lower limits for the excited electron mass are given as
$m_{e^\star}>$~200~GeV in~\cite{11}, and
$m_{e^\star}>$~306~GeV~in~\cite{12}. The 
higher limits are derived from indirect effects due to $e^\star$ exchange
in the $t$ channel, and depend on a transition magnetic coupling between
$e$ and $e^\star$. Relatively small limits
($m_{\mu^\star,\tau^\star}>$~94.2~GeV) for excited muon ($\mu^\star$) and
excited tau ($\tau^\star$) are given by the L3 experiment
at~LEP~\cite{13}. 

In this work, resonant production of an excited electron in the $s$
channel and its subsequent decay modes $e^\star \to e \gamma$,
$e^\star \to \nu W$, $e^\star \to eZ$ are considered. In
addition, we include the contributions coming from the excited electron in
the $t$ channel. The production cross section and decays of excited
electrons are calculated using the effective Lagrangian of~\cite{9}, which
depends on a compositeness scale $\Lambda$ and on free parameters $f$ and
$f^{\prime}$. We have implemented the interaction vertices into
CompHEP~\cite{comphep} for the excited electron interactions with leptons and
gauge bosons. We choose either $f=f^\prime$ or $f=-f^\prime$ in our
calculations in order to reduce the number of free parameters. For the
case $f=f^\prime$ ($f=-f^\prime$) the coupling of the photon to excited
neutrinos (electrons) vanishes.

When produced, an excited electron decays predominantly into a $W$ boson
and a neutrino, and the branching ratios are insensitive to the excited
electron mass when it is high with respect to $m_W$ or $m_Z$. We obtain the
limiting values for the branching ratios at large $m_{e^\star}$ as 0.28, 0.60
and 0.11 for the coupling $f=f^{\prime}$~=~1, in the photon, $W$ and $Z$
channels, respectively. In the case $f=-f^{\prime}$~=~--~1, the branching
ratio for the $W$ channel does not change, whilst it increases to 0.39
for the $Z$ channel. Taking $f=-f^{\prime}$~=~1 and $\Lambda$~=~1~TeV,
we find the 
total decay width of an excited electron to be 0.83~GeV and 6.9~GeV
for $m_{e^\star}$~=~500~GeV and $m_{e^\star}$~=~1000~GeV, respectively.

Excited electrons can be produced directly via the subprocess $e\gamma
\to e^{\star}\to lV$ ($V=\gamma,Z,W$) and indirectly via a
$t$-channel exchange diagram~\cite{14}. The production cross section of
excited electrons in three modes, taking $f=f^\prime$~=~1 and
$\Lambda=m_{e^\star}$, are given in Table~\ref{table4} 
%table20
for CLIC-based $e\gamma$ colliders at the 
centre-of-mass energy $\sqrt{s_{e^+e^-}}$~=~1~TeV
($\sqrt{s_{e^+e^-}}$~=~3~TeV). 
The following information can be read off~Table~\ref{table4} the following
information: the $W$ channel gives higher cross sections than the others,
but there is an ambiguity with the neutrino in this final state.
Therefore, the photon channel gives a more promising result, because of its
simple kinematics. The cross sections and the numbers of signal events are
shown in Table~\ref{table4}. For the signal and background processes we
apply a cut $p^{e,\gamma}_T>$~10~GeV for experimental identification of
final-state particles. The backgrounds to the $W$ and $Z$ decay channels
in the hadronic final states are fairly large. The backgrounds to the
photonic final states are relatively small with respect to the $W$ and
$Z$~channels.

For the signal process {$e\gamma \to e^{\star}\to
e\gamma $}, the transverse momentum $p_{T}$ distribution of the photon or
electron is peaked around the half of the mass value of the  excited
electron, as seen in~Fig.~\ref{fig2}. For the process 
$e\gamma \to e^{\star }\to \nu W \,(eZ)$, the $p_{T}$ distribution of
the $W$ boson (electron) shows a peak around
${m_{e^\star}/2}-{m^{2}_{V}/2m_{e^\star}}$, 
where $m_V$ denotes the $W$ boson
(or $Z$ boson) mass.

In order to estimate the number of events for the signal and background in
a chosen $p_T$ window, we integrate the transverse momentum distribution
around the half the mass of each excited electron
($m_{e^\star}/2-m_V^2/2m_{e^\star}$) in an interval of the transverse momentum
resolution $\Delta p_T$. Here $\Delta p_T$ is approximated as $\approx 10$
GeV for $m_{e^\star}~=~500$~GeV and $\approx 15$~GeV for $m_{e^\star}=
750$~GeV, for
a generic detector. In order to calculate the significance of the signal,
we use integrated luminosities for CLIC-based $e \gamma$ colliders of
$L$~=~10$^5$~pb$^{-1}$. In order to see the potential of CLIC-based $e
\gamma$ colliders to search for an excited electron, we define the
statistical significance $S/\sqrt{B}$, where $S$ and $B$ are the total
number of events for signal and background inside the chosen $p_T$ window,
respectively. We calculate the value of $S/\sqrt{B}$ for different
couplings, assuming $f=f^\prime$ and requiring the condition
$S/\sqrt{B}>$~5 for the signal to be observable. We find from
Table~\ref{table4} that excited electrons can be observed down to
couplings $f\simeq$~0.05 and $f\simeq$~0.1 at CLIC-based $e\gamma$
colliders with $\sqrt{s_{e^+e^-}}$~=~1~TeV and 
$\sqrt{s_{e^+e^-}}$~=~3~TeV,~respectively.

In this study, we have assumed that the excited electrons interact with
the SM particles through the effective Lagrangian~\cite{9}.
This may be a conservative assumption, because it is possible for excited
fermions to couple to ordinary quarks and leptons via contact interactions
originating from the strong constituent dynamics. In this case, the decay
widths can be enhanced~\cite{15}.

To conclude: we have presented results for excited electron production
with subsequent decays into three channels. The excited electrons
can be produced at CLIC-based $e\gamma$ colliders up to the kinematical
limit in each channel, due to the nearly flat photon energy spectrum. We
find that an excited electron with mass 500~(750)~GeV can be probed down
to the coupling $f=f^{\prime}\simeq$~0.05 at $\sqrt{s_{e^+e^-}}$~=~1~TeV. At
a CLIC-based $e\gamma$ collider with $\sqrt{s_{e^+e^-}}$~=~3~TeV the excited
electron can be probed down with couplings as low as 
$f=f^{\prime}\simeq$~0.1.

\newpage
\input{Chap6/table20.tex}
\newpage

%fig34
\begin{figure}[htbp] %[ptb]
\begin{center}
\includegraphics[width=7cm,height=6cm]{Chap6/lepto_fig3.eps}
\includegraphics[width=7cm,height=6cm]{Chap6/lepto_fig4.eps}
\includegraphics[width=7cm,height=6cm]{Chap6/lepto_fig5.eps}
\caption{Transverse momentum distribution of the photon, $W$ boson and
electron from excited electron production processes at a CLIC-based
$e\gamma$ collider with $\sqrt{s_{e\gamma}^{\rm max}}$~=~911~GeV for
different couplings $f=f^\prime$ and $m_{e^\star}$~=~500~GeV} 
\label{fig2}
\end{center}
\end{figure}

\subsection{Non-Commutative Theories}

Recent theoretical studies have demonstrated that non-commutative (NC)
quantum field theories appear naturally in the context 
of string theory in the presence of background 
fields~\cite{seiwit}. In this case, the usual space-time coordinates
no longer commute, and instead obey the relation
\begin{equation}
[\hat x_\mu, \hat x_\nu]=i\theta_{\mu\nu}\,, 
\label{NC1}
\end{equation}
where the $\theta_{\mu\nu}$ are a constant, frame-independent set of six
dimensionful parameters~\cite{rev}. The $\theta_{\mu\nu}$ may be separated
into two classes: (i) space--space non-commutativity with
$\theta_{ij}=c^B_{ij}/\Lambda_{\rm NC}^2$, 
and (ii) space-time non-commutativity
with $\theta_{0i}=c^E_{0i}/\Lambda_{\rm NC}^2$. The quantities $\hat c_{E,B}$
are two, fixed, frame-independent unit vectors associated with the NC
scale $\Lambda_{\rm NC}$.  The NC scale $\Lambda_{\rm NC}$ is most likely to be
near the string or Planck scale, which could be as low as a~TeV; it
characterizes the threshold where NC effects become apparent. Since the
two vectors $\hat c_{E,B}$ are frame-independent, they correspond to
preferred directions in space, related to the directions of the background
fields. Thus, NC theories violate Lorentz invariance, and upper limits on
such effects provide model-dependent constraints on the NC
scale~\cite{rev,sean}. Since experimental probes of NC theories are
sensitive to the directions of $\hat c_{E,B}$, the experiments must employ
astronomical coordinate systems and time-stamp their data so that 
the rotation of the Earth or the Earth's motion around the Sun, for
example, does
not wash out or dilute the effect through time-averaging.  Note that
momenta still commute in the usual way and hence energy and momentum
remain conserved quantities, as does CPT.

It is possible to construct non-commutative analogues of conventional field
theories following two approaches: Weyl--Moyal (WM)~\cite{rev} or
Seiberg--Witten (SW)~\cite{seiwit}, both of which have their own advantages
and disadvantages. In the SW approach, the field theory is expanded in a
power series in $\theta$, which then produces an infinite tower of
additional operators. At any fixed order in $\theta$ the theory can be
shown to be non-renormalizable~\cite{nonr}.  The SW construction can,
however, be applied to any gauge theory with arbitrary matter
representations.  In the WM approach, only $U(N)$ gauge theories are found
to be closed under the group algebra, and the matter content is restricted
to the (anti-)fundamental and adjoint representations.  However, these
theories are at least one-loop renormalizable, and appear to remain so
even when spontaneously broken~\cite{renorm}.  These distinctive
properties of NC gauge theories render it difficult to construct a
satisfactory non-commutative version of the SM~\cite{models}.

However, a NC version of QED is a well-defined theory in the WM approach,
and its implications for very-high-energy $e^+e^-$ colliders may be
explored. This version of NCQED differs from ordinary QED in several ways:
(i) the ordering of products of fields must be preserved through the
introduction of the star product~\cite{rev}, which absorbs the effect of
the commutation relation via a series of Fourier transforms; (ii) all
vertices pick up a Lorentz-violating phase factor that is dependent on the
momenta flowing through the vertex; (iii) NCQED takes on a non-Abelian
nature in that trilinear and quartic photon couplings are generated; and
(iv) only the charges $Q$~=~0, $\pm$~1 are allowed by gauge invariance.  We
note that propagators, however, are not modified since quadratic forms
remain unchanged when one introduces the star product.

NCQED provides a testing ground for the basic ideas behind NC quantum
field theory, and produces striking signatures in QED processes at CLIC.
The NC modifications to pair annihilation, Bhabha, M{\o}ller, and Compton
scattering, as well as $\gamma\gamma\to \gamma\gamma,e^+e^-$ have been
examined by a number of authors~\cite{ncqed}. Some of these processes
receive new diagrammatic contributions due to the non-Abelian couplings,
and all of them acquire a phase dependence due to the relative
interference of the vertex kinematic phases.  The lowest-order NC
contribution to these processes occurs via dimension-8 operators whose
scale is set by $\Lambda_{\rm NC}$.  The most striking result is that an
azimuthal-angle, $\phi$, dependence is induced in $2\to 2$ scattering
processes, since there exist the NC-preferred space-time directions,
providing a unique signature of the Lorentz violation 
inherent in these~theories.

Very-high-energy $e^+e^-$ colliders such as CLIC will allow us to probe
values of $\Lambda_{\rm NC}$ up to several~TeV provided sufficient luminosity,
$\sim$~1~ab$^{-1}$, is available~\cite{jpr}. To demonstrate this claim, we
examine the case of pair annihilation, taking the incoming $e^-$ direction
to be along the $z$-axis.  In addition to the new phases that enter the
$t$- and $u$-channel amplitudes, there is now an additional $s$-channel
photon exchange graph involving the NC-generated three-photon vertex.  
The resulting azimuthal dependence and $\cos\theta$ distribution are shown
in~Fig.~\ref{E3064_fig2} for the illustrative case $c_{02}$~=~1. Writing
$c_{01}=\cos \alpha$, $c_{02}=\sin \alpha \cos \beta$, and 
$c_{03}=\sin\alpha \sin \beta$, Fig.~\ref {E3064_fig3} 
displays the reach for
$\Lambda_{\rm NC}$ for CLIC energies for several values of~$\alpha$.

The 95\% C.L. search reaches for the NC scale in a variety of processes
are summarized in~Table~\ref{summ} for both $\sqrt{s}$~=~500~GeV and CLIC
energies. We see that these machines have a reasonable sensitivity to NC
effects and provide a good probe of such theories.  It turns out that 
M{\o}ller scattering, while sensitive only to space/space
non-commutativity, is a particularly promising process for
experimental investigation: once the 
non-commutative Feynman rules are written down, we can interpret precise
measurements of the M{\o}ller scattering cross-Section.  It may be the
interaction of choice for a possible observation of this new effect.
%!!
%fig35
\begin{figure}[t] %[htbp]
\centerline{
\includegraphics[width=7.7cm,angle=0]{Chap6/nc_thet_eegg.ps}
\hspace*{5mm}
\includegraphics[width=7.7cm,angle=0]{Chap6/nc_phi_eegg1.ps}}
\vspace*{5mm}
\caption{Shifts in the $z=\cos \theta$ and $\phi$ distributions for the 
process $e^+e^- \to \gamma \gamma$ at a 3 or 5~TeV CLIC, assuming an
integrated luminosity of 1 ab$^{-1}$. The dashed curves  
show the SM expectations while the `data' assume $c_{02}$~=~1 and 
$\Lambda_{\rm NC}=\sqrt s$. A cut of $|z|<$~0.5 has been applied in
the $\phi$~distribution.}
\label{E3064_fig2}
\end{figure}
%

~~~\\

\vspace*{15mm}

~\\

%fig36
\begin{figure}[htbp]
\centerline{
\includegraphics[width=7.7cm,angle=0]{Chap6/nc_bd_3000.ps}
\hspace*{5mm}
\includegraphics[width=7.7cm,angle=0]{Chap6/nc_bd_5000.ps}}
\vspace*{5mm}
\caption{Reach for $\Lambda_{\rm NC}$ at a 3~TeV (left) or a 5~TeV 
(right) CLIC as a function of the integrated luminosity for the process 
$e^+e^- \to \gamma \gamma$ following the notation discussed in the text}
\label{E3064_fig3}
\end{figure}
%

\input{Chap6/table21.tex}

\section{Summary}

A summary of the reach for exotic physics at CLIC, assuming a 
centre-of-mass energy of 5~TeV and an integrated luminosity of 
5~ab$^{-1}$, is given in Table~\ref{exsumm}.

\input{Chap6/table22.tex}

As we have shown in this chapter, the particular characteristics of CLIC, 
such as larger beamstrahlung and $\gamma \gamma$ backgrounds than a 
lower-energy LC, are not in general obstacles to full exploitation of 
CLIC's higher centre-of-mass energy. If the new physics is within CLIC's 
kinematic reach, CLIC will find it.

In many cases, CLIC will be able to explore in detail and unravel hints of 
new physics that might be found at the LHC. In other cases, CLIC can reach 
even far beyond the LHC, thanks to its relatively clean experimental 
conditions and its democratic production of new weakly-interacting 
particles.

